Growing Efficient Deep Networks by Structured Continuous Sparsification

We develop an approach to growing deep network architectures over the course of training, driven by a principled combination of accuracy and sparsity objectives. Unlike existing pruning or architecture search techniques that operate on full-sized models or supernet architectures, our method can start from a small, simple seed architecture and dynamically grow and prune both layers and filters. By combining a continuous relaxation of discrete network structure optimization with a scheme for sampling sparse subnetworks, we produce compact, pruned networks, while also drastically reducing the computational expense of training. For example, we achieve $49.7\%$ inference FLOPs and $47.4\%$ training FLOPs savings compared to a baseline ResNet-50 on ImageNet, while maintaining $75.2\%$ top-1 accuracy -- all without any dedicated fine-tuning stage. Experiments across CIFAR, ImageNet, PASCAL VOC, and Penn Treebank, with convolutional networks for image classification and semantic segmentation, and recurrent networks for language modeling, demonstrate that we both train faster and produce more efficient networks than competing architecture pruning or search methods.

==> poster/Makefile <==
# Paths to the programs used by this Makefile.
PDFLATEX = pdflatex --shell-escape
CP = cp
RM = rm
GREP = grep
DIFF = diff -q
TOUCH = touch

# Paths to the input and output files.
TEXFILE = growing_poster.tex
PDFFILE = growing_poster.pdf
TEXINCLUDES = $(wildcard include/*.tex)

# Paths to intermediate files that are created by the make process.
# Do not change these.
TEXLOG = $(basename $(TEXFILE)).log
AUXFILE = $(basename $(TEXFILE)).aux
FIGFILES = $(basename $(TEXFILE))-fig*
TMPINPUTS = tmp.inputs

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
.PHONY: all
all: pdf
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE) \
                 $(TEXLOG) \
		 $(FIGFILES) \
		 $(TMPINPUTS) \
                 $(PDFFILE)

